LIMDD: A Decision Diagram for Simulation of Quantum Computing Including Stabilizer States

Efficient methods for the representation and simulation of quantum states and quantum operations are crucial for the optimization of quantum circuits. Decision diagrams (DDs), a well-studied data structure originally used to represent Boolean functions, have proven capable of capturing relevant aspects of quantum systems, but their limits are not well understood. In this work, we investigate and bridge the gap between existing DD-based structures and the stabilizer formalism, an important tool for simulating quantum circuits in the tractable regime. We first show that although DDs were suggested to succinctly represent important quantum states, they actually require exponential space for certain stabilizer states. To remedy this, we introduce a more powerful decision diagram variant, called Local Invertible Map-DD (LIMDD). We prove that the set of quantum states represented by poly-sized LIMDDs strictly contains the union of stabilizer states and other decision diagram variants. Finally, there exist circuits which LIMDDs can efficiently simulate, while their output states cannot be succinctly represented by two state-of-the-art simulation paradigms: the stabilizer decomposition techniques for Clifford + $T$ circuits and Matrix-Product States. By uniting two successful approaches, LIMDDs thus pave the way for fundamentally more powerful solutions for simulation and analysis of quantum computing.

==> pics/necessity-of-reduction-rules.tex <==
\begin{tikzpicture}[
    scale=0.3,
    every path/.style={>=latex},
    every node/.style={},
    inner sep=0pt,
    minimum size=0.5cm,
    line width=1pt,
    thin,
    font=\small
    ]
    
    % nodes
    
    % nodes
    \node[draw,circle] (a1) at ( 0,-0)     {$q_2$};
    \node[draw,circle] (a2) at (0,-3) {$q_1$};
    
    \node[draw,circle,rectangle,minimum size=0.4cm] (w1) at  (-0,-6) {$1$};
    
    % edges
    \draw[dotted,bend left=-20] (a1) edge  node[left] {$1$} (a2);
    \draw[bend left=20](a1) edge  node[right] {$4$} (a2);
    
    \draw[dotted,bend left=-20] (a2) edge node[left] {$0$} (w1);
    \draw[bend left=20]       (a2) edge  node[right] {$1$} (w1);
    
    
    \node[draw,circle] (a1) at (5,-0)     {$q_2$};
    \node[draw,circle] (a2) at (5,-3) {$q_1$};
    
    \node[draw,circle,rectangle,minimum size=0.4cm] (w1) at ( 5,-6) {$1$};
    
    % edges
    \draw[dotted,bend left=-20] (a1) edge  node[left] {$1$} (a2);
    \draw[bend left=20](a1) edge  node[right] {$2$} (a2);
    
    \draw[dotted,bend left=-20] (a2) edge node[left] {$1$} (w1);
    \draw[bend left=20]       (a2) edge  node[right] {$2$} (w1);
    
    
    \node[draw,circle] (a1p) at ( 13,-0)     {$q_2$};
    \node[draw,circle] (a20) at ( 10,-3) {$q_1$};
    \node[draw,circle] (a21) at ( 16,-3) {$q_1$};
    
    \node[draw,circle,rectangle,minimum size=0.4cm] (w1) at ( 13,-6) {$1$};
    
    % edges
    \draw[dotted] (a1p) edge  node[left] {1} (a20);
    \draw[]     (a1p) edge  node[right] {2} (a21);
    
    \draw[dotted,bend left =-20] (a20) edge  node[left] {1} (w1);
    \draw[      ,bend left = 20]       (a20) edge  node[above right, xshift=-4pt] {3} (w1);
    
    \draw[dotted,bend left =-20] (a21) edge node[above left, xshift=4pt] {1} (w1);
    \draw[      ,bend left = 20]       (a21) edge  node[right] {4} (w1);
    
    
    \node[] (a2) at (2.5,-3) {$+$};
    \node[] (a2) at (7.5,-3) {$=$};
    
\end{tikzpicture}

==> preamble.tex <==
\RequirePackage{array}
\RequirePackage{color}
%\RequirePackage[utf8]{inputenc}
%\RequirePackage{graphicx}
%\RequirePackage{epigraph}
\RequirePackage{amsmath}

%\RequirePackage[ruled,vlined]{algorithm2e}
\RequirePackage{algorithm}
\RequirePackage[noend]{algpseudocode}

\RequirePackage{amssymb}
\RequirePackage{braket}
%\RequirePackage{xfrac} %for sfrac
\RequirePackage{venndiagram}

\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{thmtools}
\RequirePackage{multirow}
\RequirePackage{mleftright}
\RequirePackage{nicefrac}
%\RequirePackage{comment}
%\RequirePackage[T1]{fontenc}
%\RequirePackage{stmaryrd}
%\RequirePackage{thm-restate}
%\RequirePackage{complexity}
\RequirePackage[colorlinks,citecolor=blue!60!black!70,linkcolor=blue!60!black!70]{hyperref}%\RequirePackage{cite}
%\RequirePackage{hyperref}
%%\RequirePackage{caption}
%%\RequirePackage{subcaption}
%\RequirePackage{mathrsfs}
%\RequirePackage[english]{babel}
%%\RequirePackage{mathabx}
%%\RequirePackage{pgfplots}
\RequirePackage{calc}
\RequirePackage{todonotes}
\RequirePackage{complexity}
\RequirePackage{thm-restate}
%\RequirePackage{fdsymbol}
%\RequirePackage{eucal}
\RequirePackage{tikz}
\usepackage{blindtext}
\usetikzlibrary{shapes,backgrounds,calc,arrows,automata}
\usetikzlibrary{graphs,quotes}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{shapes,backgrounds,calc,arrows,positioning}
\usetikzlibrary{decorations.pathreplacing,calligraphy}

%\RequirePackage{verbatim}
\RequirePackage{soul}
\RequirePackage{wrapfig}
\tikzset{
  every edge/.append style = {thick}% commenting this solves the problem
}
\usepackage{empheq}



\RequirePackage[bottom,symbol]{footmisc} 
\RequirePackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}


\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.25ex \@plus 0ex \@minus .2ex}{-1ex}%
  {\normalfont\normalsize\bfseries}%
}
\makeatother


\renewcommand\mid{\;\middle|\;}




%\let\OldComment\Comment
%\renewcommand\Comment[1]{\OldComment {\footnotesize #1}}
\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$ {\footnotesize #1}}


\newlength\mytemplen
\newsavebox\mytempbox

\makeatletter
\newcommand\mybluebox{%
    \@ifnextchar[%]
       {\@mybluebox}%
       {\@mybluebox[0pt]}}

\def\@mybluebox[#1]{%
    \@ifnextchar[%]
       {\@@mybluebox[#1]}%
       {\@@mybluebox[#1][0pt]}}

\def\@@mybluebox[#1][#2]#3{
    \sbox\mytempbox{#3}%
    \mytemplen\ht\mytempbox
    \advance\mytemplen #1\relax
    \ht\mytempbox\mytemplen
    \mytemplen\dp\mytempbox
    \advance\mytemplen #2\relax
    \dp\mytempbox\mytemplen
    \colorbox{myblue}{\hspace{1em}\usebox{\mytempbox}\hspace{1em}}}
\makeatother


\definecolor{shadecolor}{cmyk}{.05,.05,0.05,0.05}
\definecolor{light-blue}{cmyk}{0.15,.15,.15,.15}
\newsavebox{\mysaveboxM} % M for math
\newsavebox{\mysaveboxT} % T for text

\newcommand*\Garybox[2][Example]{%
  \sbox{\mysaveboxM}{#2}%
  \sbox{\mysaveboxT}{\fcolorbox{black}{light-blue}{#1}}%
  \sbox{\mysaveboxM}{%
    \parbox[b][\ht\mysaveboxM+.5\ht\mysaveboxT+.5\dp\mysaveboxT][b]{\wd\mysaveboxM}{#2}%
  }%
  \sbox{\mysaveboxM}{%
    \fcolorbox{black}{shadecolor}{%
      \makebox[19em]{\usebox{\mysaveboxM}}%
    }%
  }%
  \usebox{\mysaveboxM}%
  \makebox[0pt][r]{%
    \makebox[\wd\mysaveboxM][c]{%
      \raisebox{\ht\mysaveboxM-0.5\ht\mysaveboxT+0.5\dp\mysaveboxT-0.5\fboxrule}{\usebox{\mysaveboxT}}%
    }%
  }%
}


\makeatletter
\def\blfootnote{\gdef\@thefnmark{}\@footnotetext}
\makeatother


%\RequirePackage{textgreek} % for \textchi

%\usepackage{algorithm}
%\usepackage{algpseudocode}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\declaretheorem[name=Theorem]{theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
%\newtheorem{conjecture}{Conjecture}
%\declaretheorem[name=Conjecture]{conjecture}
%\declaretheorem{definition}
%\newtheorem{problem}{Problem}
%\newtheorem{subproblem}{Problem}[problem]
%\newtheorem{solution}{Solution}[problem]
%\newtheorem{subsolution}{Solution}[subproblem]
%\newtheorem{conjecturesolution}{Solution}[conjecture]
%\newtheorem{conjecturecounterexample}{Counterexample}[conjecture]
%\newtheorem{smalldefinition}{Definition}

%\declaretheoremstyle[qed=$\diamond$]{definitionstyle}
%\theoremstyle{definitionstyle}
%\declaretheorem[style=definitionstyle]{definitions}
%


%%%% New commands for algorithmic package: Case statements
\algnewcommand\algorithmicswitch{\textbf{switch}}
\algnewcommand\algorithmiccase{\textbf{case}}
\algnewcommand\algorithmicassert{\texttt{assert}}
\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
% New "environments"
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
\algtext*{EndSwitch}%
\algtext*{EndCase}%

%




\setlength{\parskip}{7pt}
\setlength{\parindent}{0pt}


% Below: added by Tim

\usepackage{enumerate}
\newcommand{\innerprod}[2]{\langle #1 | #2 \rangle}

\newenvironment{algo}[1][Algorithm]
    {\begin{center} 
    \begin{tabular}{|p{0.9\textwidth}|} 
    \hline 
    \vspace{0.1\baselineskip} 
    \textbf{#1}\\} 
    { 
    \\\hline 
    \end{tabular} 
    \end{center} 
    \vspace{\baselineskip} 
    } 

%\theoremstyle{df}
%\declaretheorem{df}
%\theoremstyle{thm}
%\declaretheorem{thm}
%\theoremstyle{prop}
%\declaretheorem{prop}
%\theoremstyle{corollary}
%\declaretheorem{corollary}
%\theoremstyle{conj}
%\declaretheorem{conj}

%\usepackage{physics}
% package physics clashes with another package; now manually adding the
% commands needed:
%\newcommand{\expval}[1]{\langle #1 \rangle}
%\newcommand{\dyad}[1]{| #1 \rangle \langle #1 |}
%\newenvironment{smallmat}{\left[\begin{smallmatrix}}{\end{smallmatrix}\right]}
%\newcommand{\Iso}{\ensuremath{\text{Iso}}}
%\newcommand{\Stab}{\ensuremath{\text{Stab}}}
%\newcommand{\Aut}{\ensuremath{\text{Aut}}}

%\defaccr{\qmdd}{\textsf{QMDD}}
%\defaccr{\add}{\textsf{ADD}}
%\defaccr{\isoqmdd}{\textsf{LIMDD}}
%\defaccr{\limdd}{\textsf{LIMDD}}
%\defaccr{\qmdds}{\textsf{QMDD}s}
%\defaccr{\adds}{\textsf{ADD}s}
%\defaccr{\isoqmdds}{\textsf{LIMDD}s}
%\defaccr{\limdds}{\textsf{LIMDD}s}
%\defaccr{\glimdd}{\ensuremath{G}-\limdd}
%\defaccr{\glimdds}{\ensuremath{G}-\limdds}

\newcommand{\diagonal}[1]{\begin{smallmat}1 & 0 \\ 0 & #1\end{smallmat}}
\newcommand{\antidiagonal}[1]{\begin{smallmat}0 & #1 \\ 1 & 0\end{smallmat}}

%\newcommand{\tim}[1]{\textcolor{blue}{[\textbf{Tim: }#1]}}
%\newcommand{\lieuwe}[1]{\textcolor{blue}{\textbf{Lieuwe: }#1}}

%\renewcommand\index{\textsf{idx}}
%\newcommand\iso{\textsf{iso}}



%% begin appendix autoref patch [\autoref subsections in appendix](https://tex.stackexchange.com/questions/149807/autoref-subsections-in-appendix)
%\usepackage{etoolbox}
%\makeatletter
%\patchcmd{\hyper@makecurrent}{%
%    \ifx\Hy@param\Hy@chapterstring
%        \let\Hy@param\Hy@chapapp
%    \fi
%}{%
%    \iftoggle{inappendix}{%true-branch
%        % list the names of all sectioning counters here
%        \@checkappendixparam{chapter}%
%        \@checkappendixparam{section}%
%        \@checkappendixparam{subsection}%
%        \@checkappendixparam{subsubsection}%
%        \@checkappendixparam{paragraph}%
%        \@checkappendixparam{subparagraph}%
%    }{}%
%}{}{\errmessage{failed to patch}}
%
%\newcommand*{\@checkappendixparam}[1]{%
%    \def\@checkappendixparamtmp{#1}%
%    \ifx\Hy@param\@checkappendixparamtmp
%        \let\Hy@param\Hy@appendixstring
%    \fi
%}
%\makeatletter
%
%\newtoggle{inappendix}
%\togglefalse{inappendix}
%
%\apptocmd{\appendix}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
%\apptocmd{\subappendices}{\toggletrue{inappendix}}{}{\errmessage{failed to patch}}
% end appendix autoref patch




%% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
%\makeatletter
%% start with some helper code
%% This is the vertical rule that is inserted
%\newcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%
%
%\newcount\ALG@printindent@tempcnta
%\def\ALG@printindent{%
%    \ifnum \theALG@nested>0% is there anything to print
%        \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
%            % do nothing
%            \addvspace{-3pt}% FUDGE for cases where no text is shown, to make the rules line up
%        \else
%            \unskip
%            % draw a rule for each indent level
%            \ALG@printindent@tempcnta=1
%            \loop
%                \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
%                \advance \ALG@printindent@tempcnta 1
%            \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
%            \repeat
%        \fi
%    \fi
%    }%
%\usepackage{etoolbox}
%% the following line injects our new indent handling code in place of the default spacing
%\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
%\makeatother
%% end vertical rule patch for algorithmicx





\usepackage{etoolbox}

\newcommand{\algruledefaultfactor}{.75}
\newcommand{\algstrut}[1][\algruledefaultfactor]{\vrule width 0pt
depth .25\baselineskip height #1\baselineskip\relax}
\newcommand*{\algrule}[1][\algorithmicindent]{\hspace*{.5em}\vrule\algstrut
\hspace*{\dimexpr#1-.5em}}

\makeatletter
\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
    \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
    % do nothing
    \else
    \unskip
    % draw a rule for each indent level
    \ALG@printindent@tempcnta=1
    \loop
    \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
    \advance \ALG@printindent@tempcnta 1
    \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
    \repeat
    \fi
    \fi
}%

\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}

\AtBeginEnvironment{algorithmic}{\lineskip0pt}



\newcommand*\Stateh{\State \algstrut[1]}


\let\oldReturn\Return
\renewcommand\Return{\oldReturn \algstrut[1]}

\let\oldIf\If
\renewcommand\If[1]{\oldIf{#1}\algstrut[1]}

\let\oldFor\For
\renewcommand\For[1]{\oldFor{#1}\algstrut[1]}


\algnewcommand{\algorithmicgoto}{\textbf{go to}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%


\newcommand\dicke[2]{\ket{D^{#1}_{#2}}}
\newcommand{\dickebra}[2]{\bra{D^{#1}_{#2}}}

\RequirePackage{verbatim}

%\newcommand[1]{\genset}{[#1]}


==> sections/hard_to_simulate_states.tex <==
\section{A use case for \limdds}
\label{sec:very-hard-states}

In this section, we describe a family of quantum circuits we call ``Hamming weight-controlled circuits,'' which can be simulated in polynomial time using \limdds.
We analyze three popular state-of-the-art methods for quantum simulation --- matrix product states, Clifford + $T$ simulation and stabilizer rank-based methods --- and conclude that each of them is likely to need exponential time to simulate these circuits.
%
%

Given an $n$-qubit Clifford gate $C$, we define the $2n$-qubit Hamming weight-controlled Clifford gate (or HWC gate) $U_w^C$ on computational-basis states $\ket{x}, \ket{y}$ (both $n$ qubits) as
\begin{align}
    \label{eq:hamming-weight-control-gate}
    U^C_w(\ket{x} \otimes \ket{y}) = \begin{cases}
        \ket{x} \otimes C\ket{y} & \text{if } |x|=w \\
        \ket{x} \otimes \ket{y} & \text{otherwise}
	\end{cases}
\end{align}
where $|x|$ denotes the Hamming weight of bitstring $x$.
By Hamming weight-controlled Clifford (HWC) circuits,
we denote a sequence of HWC gates applied to initial state $\left(H\ket{0}\right)^{\otimes n}\otimes \ket{0}^{\otimes n}$.
\autoref{fig:weight-controlled-stabilizer-state}~(a) shows an example.
We refer to the output state as a HWC state.
%


The \limdd representing a HWC state containing $t$ HWC gates has width $t+1\leq n+1$, and therefore has $\mathcal O(n^2)$ nodes.
\autoref{fig:weight-controlled-stabilizer-state}(b) shows an example.
First, the division of length-$n$ bitstrings depending on the Hamming weight is a known construction for BDDs~\cite{bryant86}, yielding a DD for the control register whose width which cannot exceed $n+1$.
The target register consists of a series of states $C_w \ket{0}^n$, each of which is a stabilizer state because $C_w$ is a Clifford operation.
Since Pauli-\limdds can represent $n$-qubit stabilizer states with $n$ nodes (\autoref{sec:exponential-separations}), the resulting \limdd for the entire HWC state has polynomially-many nodes.
To simulate this circuit, we build a \limdd for each individual Hamming weight-controlled Clifford gate in the Clifford circuits $C_w$.
These \limdds have polynomial size and look similar to those in \autoref{fig:weight-controlled-stabilizer-state}.

%

\begin{figure}[b!th]
	\centering
	\includegraphics[width=\textwidth]{pics/weight-controlled-stabilizer-state-2.pdf}
	\caption{
        \textbf{(a)} A ``Hamming weight-controlled Clifford circuit'' on $3+3$ qubits with input state $\ket{0}^{\otimes 3} \otimes \ket{0}^{\otimes 3}$. 
        The depicted circuit consists of three controlled-Clifford gates, where the Clifford $C_w$ is only applied if the Hamming weight of the control register equals $w$ see also eq.~\eqref{eq:hamming-weight-control-gate}.
        \textbf{(b)} A Pauli-\limdd for the output state of the circuit in (a), where the colored blocks represent Pauli-\limdds for the states $C_w \ket{0}^{\otimes 3}$.
        The edges which originate in the control-register-part of the \limdd point to the top node of three different branches, each representing a constant Hamming weight of the control qubits (edge weights are all $\id$; recall dashed/solid lines represent low/high edges).
        The branch in the target-register-part corresponding to Hamming weight $w$ represents the state $C_w \ket{0}^{\otimes 3}$, which is a stabilizer state.
        We note that stabilizer states are represented by a polynomially-large \limdd (see \autoref{sec:exponential-separations}) while the width of the control-register-part of the \limdd can never exceed the possible number of Hamming weights on length-$n$ bitstrings, i.e. ${n \choose 2} = O(n^2)$.
        Consequently, Pauli-\limdds represent all Hamming weight-controlled Clifford circuits using only polynomially-many nodes.
    }
	\label{fig:weight-controlled-stabilizer-state}
\end{figure}

In order to investigate the hardness of HWC circuits for general stabilizer rank methods, we now argue that some HWC states have high stabilizer rank.
To this end, we employ the heuristic algorithm from \cite{bravyi2016trading} (explained in more detail in \cite{calpin2020exploring}) for searching for the stabilizer rank of Dicke states $\dicke{n}{w}$, which are equal superpositions of computational basis states with a given Hamming weight:
\[
    \dicke{n}{w} \defn \sum\limits_{\substack{x \in \{0, 1\}^n, \\|x| = w}} \ket{x}
    .
\]
To see that there exist HWC states $\ket{\phi}$ which have stabilizer rank $\chi(\ket{\phi})$ at least as large as the stabilizer rank $\chi(\dicke{n}{w})$ of Dicke states, consider the HWC circuit consisting of the single gate $U_w^C$ where $C$ is the Pauli $X$ gate on the least significant qubit in the target register.
The resulting state is
\begin{equation}
    \label{eq:dicke}
    \ket{\phi} =
    \sum_{k=0,k\ne w}^n \dicke{n}{k}\otimes \ket{0}^{\otimes n} + \dicke{n}{w}\ket{0\ldots 01}
\end{equation}
By measuring the target register in the computational basis, the resulting control register state is $\dicke{n}{w}$ upon obtaining output $\ket{0\ldots 01}$.
Since computational-basis measurements cannot increase the stabilizer rank, we find $\chi(\ket{\phi}) \geq \chi(\dicke{n}{w})$.

\todo[inline]{@Tim: Why is $\chi(\dicke 95)\leq 11$ the theoretical upper bound? I suppose it's something like $\chi(\dicke nw)\leq \chi(\dicke{n-1}{w})+\chi(\dicke{n-1}{w-1})$? It seems plausible that should hold... $\dicke{n}{w}=\ket{0}\dicke{n-1}{w}+\ket{1}\dicke{n-1}{w-1}$, ok, I believe; at least we should explain it. -LV}
\todo[inline]{@Tim: It says we have not investigated $w>\ceil{\frac n2}$, but I think it should be that we should not investigate $w>\floor{\frac n2}$. Agree? Or why is the $\dicke 95$ in the table?}

The heuristic algorithm follows a simulated annealing approach: on input $n,w $ and $\chi$, it performs a random walk through sets of $\chi$ stabilizer states.
It starts with a random set $V$ of $\chi$ stabilizer states on $n$ qubits.
In a single `step', the algorithm picks one of these states $\ket{\psi} \in V$ at random, together with a random $n$-qubit Pauli operator $P$, and replaces the state $\ket{\psi}$ with $\ket{\psi'} := c(\id + P)\ket{\psi}$ with $c$ a normalization constant (or repeats if $\ket{\psi'} = 0$), yielding a new set $V'$.
The step is accepted with certainty if $F_V < F_{V'}$, where $F_V:= |\dickebra nw \Pi_V \dicke{n}{w}|$ with $\Pi_V$ the projector on the subspace of the $n$-qubit Hilbert space spanned by the stabilizer states in $V$.
Otherwise, it is accepted with probability $\exp(-\beta (F_{V'} - F_V))$, where $\beta$ should be interpreted as the inverse temperature.
The algorithm terminates if it finds $F_V = 1$, implying that $\dicke{n}{w}$ can be written as linear combination of $V$, outputting the number $\chi$ as (upper bound on) the stabilizer rank.
For a fixed $\chi$, we use identical values to Bravyi et al. \cite{bravyi2016trading} and vary $\beta$ from $1$ to $4000$ in $100$ steps, performing $1000$ steps at each value of $\beta$.
%
%
%
%
See \cite{githubrepo} for our open-source implementation.
\todo[inline]{@Tim: Is the algorithm exact? Does it decide whether $\bra{D_w^n}\Pi_V\dicke nw=1$ with certainty, or only up to numerical accuracy? I imagine you are doing Gaussian elimination, which is infamous for producing rounding errors. -LV, VD}


We provide the results of our numerical runs in \autoref{table:stabilizer-rank-search}.
Since our approach is based on using heuristic algorithms to find as low as possible an upper bound \todo[inline]{Or ``to find an as low as possible upper bound''? -LV}on the stabilizer rank, and not a lower bound, by construction we cannot guarantee any statement on the scaling of the rank itself.
Our approach could only have provided evidence that Dicke states have very slowly growing rank, thereby providing evidence that stabilizer-rank methods can simulate HWC states efficiently.
%
However, this is not what we observe; at the very least we can say that, if Dicke states have low stabilizer rank, then current state-of-the-art methods do not succeed in finding the corresponding decomposition.
Although further research is needed for a definitive answer, these numerics strengthen our confidence that \limdds can simulate HWC circuits faster than stabilizer-rank based methods.


